Spin nematic states in spin-1 antiferromagnets with easy-axis anisotropy

It is well known that spin nematic phases can appear in either frustrated magnets or in those described by Hamiltonians with large exotic non-Heisenberg terms like biquadratic exchange. We show in the present study that non-frustrated spin-1 1D, 2D and 3D antiferromagnets with single-ion easy-axis anisotropy can show nematic phases in strong magnetic field. For 1D case we support our analytical results by numerical ones.

==> com.tex <==
\newcommand{\half}{\dfrac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}
\newcommand{\sqhalf}{\frac{1}{\sqrt{2}}}
\newcommand{\dNN}{\dfrac{1}{N}}

\newcommand{\beq}{\begin{eqnarray}}
\newcommand{\eeq}{\end{eqnarray}}

\newcommand{\bfig}{ \left. \begin{array}{l} }
\newcommand{\bfigor}{ \left\{ \begin{array}{ll} }
\newcommand{\efig}{ \end{array} \right. }

\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}


\newcommand{\delT}{\, \delta_{T}}


\newcommand{\ii}{\imath}
\newcommand{\vv}{\Big|}

\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}

\newcommand{\cH}{{\cal H}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cF}{{\cal F}}
\newcommand{\bS}{{\bf S}}
\newcommand{\tilh}{\tilde{h}}

\newcommand{\non}{\nonumber}

\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\w}{\omega}
\newcommand{\W}{\Omega}
\newcommand{\e}{\epsilon}
\newcommand{\p}{\rho}
\newcommand{\sig}{\sigma}
\newcommand{\Sig}{\Sigma}
\newcommand{\tSig}{\tilde\Sigma}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\Th}{\theta}


\newcommand{\bSig}{\overline{\Sig}}
\newcommand{\bPi}{\overline{\Pi}}
\newcommand{\bF}{\overline{F}}
\newcommand{\bD}{\widetilde{D}}
\newcommand{\waveS}{\widetilde{S}}


\newcommand{\krest}{\dagger}
\newcommand{\akrest}{a^\krest}
\newcommand{\bkrest}{b^\krest}
\newcommand{\akr}{\akrest}
\newcommand{\bkr}{\bkrest}
\newcommand{\kk}{{\bf k}}
\newcommand{\qq}{{\bf q}}
\newcommand{\pp}{{\bf p}}
\newcommand{\kkk}{{{\kk}_0}}
\newcommand{\ppp}{{{\pp}_0}}
\newcommand{\kz}{{k_0}}

\newcommand{\ckr}{c^\krest}
\newcommand{\dkr}{d^\krest}



\newcommand{\RR}{{\bf R}}

\newcommand{\mkk}{{\bf -k}}
\newcommand{\mpp}{{\bf -p}}

\newcommand{\sx}{\widehat{\sigma}_x}
\newcommand{\sy}{\widehat{\sigma}_y}
\newcommand{\sz}{\widehat{\sigma}_z}

\newcommand{\Par}{\parallel}
\newcommand{\Perp}{\perp}
